Composability in Watermarking Schemes

Software watermarking allows for embedding a mark into a piece of code, such that any attempt to remove the mark will render the code useless. Provably secure watermarking schemes currently seems limited to programs computing various cryptographic operations, such as evaluating pseudorandom functions (PRFs), signing messages, or decrypting ciphertexts (the latter often going by the name ``traitor tracing''). Moreover, each of these watermarking schemes has an ad-hoc construction of its own. We observe, however, that many cryptographic objects are used as building blocks in larger protocols. We ask: just as we can compose building blocks to obtain larger protocols, can we compose watermarking schemes for the building blocks to obtain watermarking schemes for the larger protocols? We give an affirmative answer to this question, by precisely formulating a set of requirements that allow for composing watermarking schemes. We use our formulation to derive a number of applications.

==> definitions_sketch.tex <==
\section{Definitions Sketch}


\paragraph{Definition 1: CPA/PRF/CCA Watermarking Compatible Reduction}

Suppose a primitive $P$ is constructed blackboxly from primitive $P_1, P_2, \cdots, P_k$:
%then for each $i \in [k]$

Each primitive $P$ consists of the following algorithms, w.l.o.g.:
\begin{itemize}
    \item $\KeyGen(1^\lambda) \to (\sk, \pk)$
    
    \item $\SecAlg(\sk, \cdot) $

    \item $\PubAlg(\pk, \cdot)$
    
\end{itemize}




Suppose that $P=(\KeyGen,\PubAlg,\SecAlg)$ and the primtive $P_i = (\KeyGen_i,\PubAlg_i,\SecAlg_i)$ all have security defined via a watermarking compatible game, and that there is a "watermarking compatible” proof of security for $P=(\KeyGen,\PubAlg,\SecAlg)$ from the assumed security of the $P_i$. This is a reduction mapping an adversary A for $P$ into adversaries $\A_i$ for $P_i$ such that:
If $\A$ has non-negligible advantage, then there must be some $i$ such that $\A_i$ has non-negligible advantage.



\paragraph{Watermarking Compatible Reduction}
\begin{itemize}
    \item Let adversary $\A = (\A^1, \A^2)$ be the adversary for primitive $P$; let $\A_i$ be the adversary for primitive $P_i$.

    \item $\A_i$ receives an abitrary leakage $\tildesk_i \gets L(\sk_i)$ on the secret key $\sk_i$ from the challenger. 
    
    
    \item $\A_i$ prepares $(\sk_j, \pk_j) \gets \KeyGen_j(1^\lambda) $ for all $j \neq i$ and generates leakage $\tildesk_j$ from $\sk_j$ for all $j\neq i$.
$\A_i$ sends all $\{\pk_\ell, \tildesk_\ell\}_{\ell \in [k]}$
to $\A_1$.

\item $\A^1$ generates a state $\st$ and gives it to $\A^2$.

    \item  $\A_i$ simulates the security game for $P$ with $\A$: for any queries in the game, if $\sk_i$ is required to compute the answer for the query, $\A_i$ queries the challenger for $P_i$ on the oracle $\SecAlg(\sk,\cdot)$.
    Otherwise, if only $\sk_j, j\neq i$ are needed, $\A_i$ answers them by itself.

    \item \jiahui{still need to capture what $\A_i$ does in order to "win" according to $\A$'s behavior. Here is my take:}
    $\A'$ computes a predicate $F_i$ on input of $\A^2$'s final answer and its queries, and gives it to the challenger of primitive $P_i$.   
\end{itemize}

\paragraph{Example: CPA security to weak-PRF}



\paragraph{Example: CCA security to MAC}
\begin{itemize}
    \item MAC adversary $\A'$ receives $\tildesk^*$ on MAC secret key. Samples $\tildesk_{2}$ for encryption on its own. Gives all the leakages to the CCA adversary $\A$.

    \item The first stage CCA adversary $\A^1$ generates a state $\st$ and gives it to the second stage $\A^2$. 

    \item The second stage adversary $\A^2$' (which does not get anything from $\A^1$') simply runs
    $\A^2$ and answers its queries:
    \begin{itemize}
        \item For any encryption query to oracle $\Enc(\sk_1, sk_2, \cdot)$: $\A_2'$ computes the encryption part with $\sk_1$ and queries the MAC-signing oracle $\sign(\sk_1, \cdot)$ to compute the part that reuires $\sk_1$. 

        \item For any decryption query to oracle $\Dec(\sk_1, sk_2, \cdot)$: similarly, $\A^2$' queries the MAC-verification oracle $\ver(\sk_1, \cdot)$ to compute the part that requires $\sk_1$.

        
    \end{itemize}

    \item $\A_2'$ will pass on any \emph{decryption} query from $\A_2$ that did not come from its encryption query, but the part that requires MAC-verification passes $\ver(\sk_1,\cdot)$, to the MAC challenger as its answer.

    \item If $\A^2$ wins the CCA game with advantage $\epsilon$ and generates at least a decryption query as above, then $\A^{2'}$ wins the MAC game with same advantage.
\end{itemize}

\begin{remark}
    If $\A^2$ does not query on any decryption queries that did not come from encryption queries, then $\A^2$ can be used to break the underlying PRF security.
\end{remark}

\jiahui{ISSUE: a watermarking scheme based on this may require the EXTRACT algorithm to know the secret key of the underlying functionality. Did this definition appear in past works?

Extract algorithm does not require "knowing the secret key of the functionality" because the underlying functionalities in existing works do not require "secret key" to run evaluation of a program:
Example: CPA-secure PKE encryption; signatures;

In our case, these following functionalities require "secret key of the functionlity" to evaluate: CPA secure symmetric key decryption, CCA-secure PKE/SKE.


See \cite{goyal2021beyond}: Defined Traceable PRFs
}




==> incompatible_watermark_sig.tex <==
\section{Definition 2: Non-Waternarking-Compatible (Incompressible) Type Definition}

\begin{itemize}
    \item Stage 1 adversary $\A_1$ receives a leakage $\tildesk$ on $\sk$. Produces a size bounded state $\st$ to stage 2 adversary $\A_2$.

    \item $\A_2$ produces a sequence of input-output pairs $\{(x_\ell, y_\ell)\}_{\ell}$ such that 
    $\vert \sum_\ell x_\ell \vert > \st$. 


    \item Challenger checks if $x_\ell, y_\ell \in R$ for some relation $R$, for all $\ell$. If yes, $\A$ wins; else no.
    
\end{itemize}


\paragraph{Construction: Watermarking Signatures from "Incompressibly Unlearnable Functions"}

Building blocks:
Constrained signature $(\CSig.\sign, \CSig.\constrain, \CSig.\ver) $ + watermarkable imcompressible function $f$.

\begin{itemize}
    \item $\KeyGen(1^\lambda)$: run $\CSig.\KeyGen(1^\lambda) \to (\CSig.\sk, \CSig.\vk)$;
     %For constant function $f_0: \{0,1\}^* \to 0^n$, compute $\sk_f \gets \CSig.\constrain(\sk, f_0)$.
    
    \item $\watermark(\sk)$
    Sample watermarkable imcompressible function $f \gets \mathcal{F}$. Compute $\tilde{f} \gets \watermark(f)$;
     Compute $\sk_f \gets \CSig.\constrain(\sk, f)$.
     Let watermarked signing key be $(\sk_f, \tilde{f})$
    
    \item $\sign(\sk, m)$:  $\sk = (\sk_f, f)$. Compute $y = f(m)$. Compute $\sigma = \CSig.\sign(\sk_f, m, y)$. 

    \item  $\ver(\vk, m, \sigma)$


    
    
\end{itemize}

==> outline.tex <==
\section{TODO}

\begin{itemize}
    \item Prelims: PRF, SKE, PKE watermarking defs, CCA normal security (and mention CPA security in one sentence)
    
    \item discuss the limitations: WMSetup generate xk and sk altogether; private extraction

    \item add all descriptions to algorithms syntax

    \item add to the proof of general reduction about computational simulation

    \item change the CCA SKE proof

    \item discussion on FE construction

    \item change all wording in proofs to deal with the outer probability
\end{itemize}

==> reduction_type2.tex <==
\subsection{Watermarking-Compatible Construction Type 2}

We introduce a second type of watermarking compatible construction and reduction. The major difference is that in watermarking-compatible construction Type 2, the algorithm $\KeyGen(1^\lambda)$ will not compute $P_i.\KeyGen(1^\lambda)$ for all $i \in [k]$, but only a subset of $[k]$; the rest of the underlying primitives will have their keys generated "freshly" upon every run of $\SecAlg$ or $\PubAlg$.

\jiahui{construction where some of the primitives are generated online during Eval algo}

Suppose a cryptographic primitive $P$ is constructed blackboxly from primitives $P_1, P_2, \cdots, P_k$ in the following way. Let $\cS$ be some fixed subset of $[k]$ defined in the construction.

\begin{description}
      \item $\KeyGen(1^\lambda) \to (\sk, \pk)$: 
      \begin{enumerate}
        \item compute $(\sk_i, \pk_i, \xk_i, \mk_i) \gets P_i.\KeyGen(1^\lambda)$ for all $i \in \cS$, where $\cS$ is a fixed subset of $[k]$.
        \item output $\sk = (\{\sk_{i}\}_{i \in \cS}); \pk = (\{\pk_{i}\}_{i \in \cS})$.
    \end{enumerate}
       \item $\SecAlg(\sk, \pk, x \in \sX) \to y \in \sY_s:$ is an algorithm that 
       \begin{enumerate}
         \item   uses $P_i.\SecAlg(\sk_i,\pk_i, \cdot), i \in \cS$ as subroutines.
         \item uses $P_i.\PubAlg(\pk_i, \cdot), i \in \cS$ as subroutines.
           \item computes $(\sk_j, \pk_j) \gets P_j.\KeyGen(1^\lambda)$ for some $j \notin \cS$; include these $\{\pk_j\}_j$ generated as part of the output.

    
           
       \end{enumerate}
     
     
    \item $\PubAlg(\pk, x \in \sX) \to y \in \sY_p:$ 
     is an algorithm that  \begin{enumerate}
         \item uses $P_i.\PubAlg(\pk_i, \cdot), i \in \cS$ as subroutines.
           \item computes $(\sk_j, \pk_j) \gets P_j.\KeyGen(1^\lambda)$ for some $j \notin \cS$; include these $\{\pk_j\}_j$ generated as part of the output.       
       \end{enumerate}

\end{description}


\paragraph{Watermarking-Compatible Reduction Type 2}
Let adversary $\A = (\A^1, \A^2)$ be the adversary for primitive $P$.

First consider doing reduction to $P_i$ for $i \in \cS$:
\begin{enumerate}
    \item Let $j = 1, \cdots, |\cS|$.
    
    \item Consider doing reduction to $P_i$ for the $j$-th $P_i \in \cS$; let $\A_i = (\A_i^1, \A_i^2)$ be the two-stage adversary for primitive $P_i$.

    \item $\A_i$ receives public key $\pk_i$ and a leakage $\tildesk_i \gets L_i(\sk_i)$ on the secret key $\sk_i$ from the challenger, where the leakage function $L_i$ is specified by the security game $G_{P_i}$.
    
    
    \item $\A_i$ prepares $(\sk_j, \pk_j) \gets \KeyGen_j(1^\lambda) $ for all $j \neq i, j \in \cS$ and generates leakage $\tildesk_j \gets L_j(\sk_j)$ for all $j\neq i, j \in \cS$, where the leakage function $L_j$ is specified by the security game $G_{P_j}$.
$\A_i$ sends all $(\{\pk_j, \tildesk_j\}_{j \in \cS})$
to $\A_1$.

%\item $\A^1$ generates a state $\st$ and gives it to $\A^2$.

    \item  $\A_i$ simulates the security game $G_P$ for $P$ with $\A$, while being the adversary in game $G_{P_i}$: 
    \begin{itemize}
        \item  For any (admissible) queries in the game $G_P$, if $\sk_i$ is required to compute the answer for the query, $\A_i$ can query the challenger for $P_i$ on the oracle $\SecAlg(\sk_i,\cdot)$\footnote{That means, the security game $G_{P_i}$ allows an adversary to make such queries.}. To answer the entire query, $\cA_i$ may finish the rest of the computation using $\{\sk_j\}_{j\neq i}$.

        \item If only $\{\sk_j\}_{j\neq i}$ are needed, $\A_i$ answers them by itself.

               % \item $\A$ does \emph{not} record $\A^1$'s queries.

       

        \item $\A^1$ generates a state $\st$ and gives it to $\A^2$. $\A_i$ is informed that $\A$ has entered stage $\A^2$ and $\A_i$ also enters its second stage $\A_i^2$.

     \item $\A_i^2$ does \emph{not} get to see any of $\A^1$'s queries.

        \item $\A_i^2$ continues to provide the same oracles needed for game $G_P$ and answer $\A^2(\st)$'s queries using the above strategy. $\A_i^2$ also records all  of $\cA^2$'s queries. 
    \end{itemize}
    
   
   

    \item \jiahui{still need to capture what $\A_i$ does in order to "win" according to $\A$'s behavior. Here is my take:}
    $\A_i$ computes a function $f_i$ on input of $\A^2$'s final answer and its queries, and gives it to the challenger of primitive $P_i$.

    \item If $\A_i$ does not succeed in winning $G_{P_i}$; increment $j := j+1$ and go to step 2. 
\end{enumerate}

Next consider reduction when $i \notin \cS:$
\begin{enumerate}
    \item Let $j = 1, \cdots, k-|\cS|$.
    
    \item Consider doing reduction to $P_i$ for the $j$-th $P_i \notin \cS$; let $\A_i = (\A_i^1, \A_i^2)$ be the two-stage adversary for primitive $P_i$.

    \item $\A_i$ receives public key $\pk_i$ from the challenger. 
    
    
    \item $\A_i$ prepares $(\sk_\ell, \pk_\ell) \gets P_\ell.\KeyGen(1^\lambda) $ for all $\ell \in \cS$ and generates leakage $\tildesk_\ell$ from $\sk_\ell$ for all $\ell \in \cS$.
$\A_i$ sends all $(\{\pk_\ell, \tildesk_\ell\}_{\ell \in \cS})$
to $\A_1$.


    %$\A_i$ prepares $(\sk_j, \pk_j) \gets \KeyGen_j(1^\lambda) $ for all $j \neq i$ and generates leakage $\tildesk_j$ from $\sk_j$ for all $j\neq i, j \in \cS$.
%$\A_i$ sends all $(\{\pk_i\}_{i \in [k]},\{\tildesk_\ell\}_{\ell \in \cS})$ to $\A_1$.



    \item  $\A_i$ simulates the security game $G_P$ for $P$ with $\A$: 
    \begin{itemize}
        \item  For any (admissible) queries in the game $G_P$, if $\sk_i$ is required to compute the answer for the query, $\A_i$ can query the challenger for $P_i$ on the oracle $\SecAlg(\sk_i,\cdot)$. To answer the entire query, $\cA_i$ may finish the rest of the computation using $\{\sk_j\}_{j\neq i}$.

        \item If only $\{\sk_j\}_{j\neq i}$ are needed, $\A_i$ answers them by itself.

       % \item $\A$ does \emph{not} record $\A^1$'s queries.
   

        \item $\A^1$ generates a state $\st$ and gives it to $\A^2$. $\A_i$ is informed that $\A$ has entered stage $\A^2$ and $\A_i$ also enters its second stage $\A_i^2$.

     \item $\A_i^2$ does \emph{not} get to see any of $\A^1$'s queries.

        \item $\A_i^2$ continues to provide the same oracles needed for game $G_P$ and answer $\A^2(\st)$'s queries using the above strategy. $\A_i^2$ also records all  of $\cA^2$'s queries. 
    \end{itemize}
    
   
   

    \item \jiahui{still need to capture what $\A_i$ does in order to "win" according to $\A$'s behavior. Here is my take:}
    $\A_i$ computes a function $f_i$ on input of $\A^2$'s final answer and its queries, and gives it to the challenger of primitive $P_i$.

    \item If $\A_i$ does not succeed in winning $G_{P_i}$; increment $j := j+1$ and go to step 2. 
\end{enumerate}



The reduction guarantees that if the advantage of $\A$ winning the game is non-negligible, i.e. $\Pr[G_P(1^\lambda,A) = 1] \geq \eta+\delta$ where $\eta$ is the trivial winning probability and $\delta$ is non-negligible in $\lambda$, then there exists some $i \in [k]$ such that $\A_i$ wins $G_{P_i}$ with some non-negligible advantage.

==> watermark_compatible_type2.tex <==
\subsection{Watermark-Compatible Type 2}
\jiahui{One primitive is sampled *online* or temporarily. generated freshly during every run of the main algortihm (with aalready fixed pk,sk) }
\paragraph{Hybrid Encryption (KEM)}
A CCA-secure hybrid encryption $\he = (\he.\KeyGen, \he.\Enc, \he.\Dec$  can be built from a CCA-secure secret key encryption scheme $\ske = (\ske.\KeyGen, \ske.\Enc, \he.\Dec)$ and a CCA-secure public key encryption $\pke = (\pke.\KeyGen, \pke.\Enc, \pke.\Dec)$ as follows:

\begin{itemize}
    \item $\he.\KeyGen(\lambda):$ compute  $(\pk_1, \sk_1) \gets \pke.\KeyGen(\lambda)$. %$\sk_1\gets \ske.\KeyGen(\lambda)$.

    \item $\he.\Enc(\pk_1, m)$: compute $\sk_2 \gets \ske.\KeyGen(\lambda)$; then compute $\ct_1 \gets \pke.\Enc(\pk_1, \sk_1)$; compute $\ct_2 \gets \ske.\Enc(\sk_2, m)$. Output $\ct = (\ct_1, \ct_2)$.

    \item $\he.\Enc(\sk_1, \ct)$: parse $\ct = (\ct_1, \ct_2)$; compute $\sk_1' \gets \pke.\Dec(\sk_1, \ct_1)$ and then $m' \gets \ske.\Dec(\sk_2, \ct_2)$. Output $m'$.

    \item Additional Algorithm decrypting using just $\sk_2$ 
\end{itemize}

\paragraph{Watermarking Compatible Reduction}
When we do reduction from a watermarked $\he$ scheme to the watermarking security of a $\pke$ scheme, we can allow the following to happen:

\begin{itemize}
    \item Suppose there exists adversary $\A$ against watermarking security of CCA-secure $\he$ (\jiahui{define what this means}), then we can build reduction $\cB$ as follows.

    \item $\cB$ receives leakage of the $\pke$'s secret key $\tildesk_1$ and $\pk_1$ from challenger.

    \item $\cB$ gives $\tildesk_1, \pk_1$ to $\A$. $\A$ produces a leakage $P$.

    \item By assumption $P$ should win the CCA-security game, in which encryption/decryption oracles are given $\Enc(\pk_1,\cdot),\Dec(\sk_1,\cdot)$ %and $\Dec(\cdot)$ can be simulated by knowing the $\sk_2$ used in upon encryption of the ciphertext to be decrypted. \jiahui{be more specific on what this HE-CCA secure game looks like. How does the Decryption oracle know which $\sk_2$ was used on this ciphertext?}
    $\cB$ will make a program $P' = P^{\Enc(\pk_1,\cdot), \Dec(\cdot)}$ to win the CCA-secure PKE watermarking game.

    \item given a program $P'$, the $\extract$ algorithm will run program $P'$ and extract watermark from it. \jiahui{When running $P'$, do we have to give oracle $\Dec(\sk_1,\cdot)$? Becasue $P'$ is supposed to break CCA-security of $\pke$. }
   
    \item If one cannot extract watermark from $P'$, then can use $P'$ to break **CCA security ** of SKE (instead of watermarking security). 

    \item Thus, the $\he$ watermarking scheme does not require the extraction to have the secret key for $\pke$, even though the watermarking for $\pke$ does. 
\end{itemize}


\jiahui{more schemes like Hybrid encryption?
To summarize: there is really only one key in the main functionality, the rest of the functionalities are "sampled online"}
